Step by Step to Fairness: Attributing Societal Bias in Task-oriented Dialogue Systems

Recent works have shown considerable improvements in task-oriented dialogue (TOD) systems by utilizing pretrained large language models (LLMs) in an end-to-end manner. However, the biased behavior of each component in a TOD system and the error propagation issue in the end-to-end framework can lead to seriously biased TOD responses. Existing works of fairness only focus on the total bias of a system. In this paper, we propose a diagnosis method to attribute bias to each component of a TOD system. With the proposed attribution method, we can gain a deeper understanding of the sources of bias. Additionally, researchers can mitigate biased model behavior at a more granular level. We conduct experiments to attribute the TOD system's bias toward three demographic axes: gender, age, and race. Experimental results show that the bias of a TOD system usually comes from the response generation model.

==> sections/abstract.tex <==
\begin{abstract}
% Researchers have shown considerable improvements in task-oriented dialogue (TOD) by training TOD systems with pretrained large language models (LLMs) in an end-to-end manner. However, the problems that come thick and fast are the bias leveraged by LLMs and error propagation issues in the end-to-end framework. 
% To teardown and solve the problems, we propose a new diagnosis method shedding light on TOD systems; 
% the proposed method addresses the accountability of each module toward bias in end-to-end TOD systems. 
% With the experimental results, we found that the bias attribution of each module mostly comes from the response generation module. 
Recent works have shown considerable improvements in task-oriented dialogue (TOD) systems by utilizing pretrained large language models (LLMs) in an end-to-end manner. However, the biased behavior of each component in a TOD system and the error propagation issue in the end-to-end framework can lead to seriously biased TOD responses. Existing works of fairness only focus on the total bias of a system. In this paper, we propose a diagnosis method to attribute bias to each component of a TOD system. With the proposed attribution method, we can gain a deeper understanding of the sources of bias. Additionally, researchers can mitigate biased model behavior at a more granular level. We conduct experiments to attribute the TOD system's bias toward three demographic axes: gender, age, and race. Experimental results show that the bias of a TOD system usually comes from the response generation model.
\end{abstract}

==> sections/bias_in_tod_systems.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Bias in TOD Systems}
\label{sec:tod}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%As mentioned in Section \ref{sec:intro}, we want to find out why the model has a disparity in generated responses given different demographics. Furthermore, we want to decompose the bias contributions of each module in TOD. To accomplish both of these purposes, we propose a diagnosis method to help us measure the accountability for each module in terms of bias.

In this section, we propose a diagnosis method to attribute the bias to the components of TOD systems. We first introduce the architecture of common TOD systems in Section~\ref{subsec:task-oriented_dialogue}. We then formally define the fairness metric in Section~\ref{subsec:definition_of_fairness}. The proposed diagnosis method is described in Section~\ref{subsec:proposed_method}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Task-Oriented Dialogue (TOD) System}
\label{subsec:task-oriented_dialogue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As shown in Figure~\ref{fig:example}, a TOD system consists of three components: API call model, database, and response generation model. Once a user utterance is provided, the API call model generates an API call according to the user utterance. Then, the TOD system converts the API call to a database search command and searches the necessary data from the database. At last, the response generation model generates the response according to the user utterance, the API call, and the database results.

%In this section, we first introduce the TOD we used to train models. We employed the similar TOD framework to \cite{chen2021teaching}. 
%As \autoref{fig:example}, the framework could be decomposed into several models. First, the dialogue state model generates API call given user utterances. The database generates the API response if a successful API call is made. Finally, the response generation module generates the final system response for the user, given the concatenation of user utterance, API call, and API response.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Definition of Fairness}
\label{subsec:definition_of_fairness}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
To measure the bias of TOD systems, we formally define the fairness metric.  We utilize the concepts of helpfulness \cite{sun2022computation} and perturbation \cite{qian2022perturbation} to define the metric. That is, the model responses should have similar helpfulness for original and demographic-perturbed user utterances. We use BLEU \cite{papineni-etal-2002-bleu} score of the model response and the ground truth to evaluate helpfulness. For example, the response of the user utterance: ``I would like to find a movie for my \textit{mom}.'' should have similar helpfulness to the response of the user utterance: ``I would like to find a movie for my \textit{dad}.'' According to this, we propose a newly designed fairness metric (Equation~\ref{eqn:fairscore}). Note that fairscore refers to our newly designed fairscore metric in the rest of the paper, not the fairscore proposed by existing works. 
\begin{equation}
    \label{eqn:fairscore}
    F_{S} = \frac{|BLEU(f_t(u_t), g_t) - BLEU(f_t(\widetilde{u_t}), \widetilde{g_t})|}{BLEU(f_t(u_t), g_t)}
\end{equation}
We denote the TOD system as $f_t$, original user utterances as $u_t$, original responses as $f_t(u_t)$, and original ground truths as $g_t$. Perturbed user utterances and ground truths are denoted as $\widetilde{u_t}$ and $\widetilde{g_t}$, respectively. As aforementioned, we expect a fair model to generate responses with similar helpfulness for original and perturbed user utterances. More specifically, we calculate the absolute value of the difference between original helpfulness $BLEU(f_t(u_t, g_t))$ and perturbed helpfulness $BLEU(f_t(\widetilde{u_t}), \widetilde{g_t})$, and normalize the helpfulness change to original helpfulness to evaluate the bias of a TOD system.
\begin{figure*}[t]
    \centering
    \includegraphics[ width = \linewidth]{pics/framework.pdf}
    \caption{The proposed framework, we input both original and perturbed user utterance and measure the bias attribution of each module by changing the module step by step.}
    \label{fig:framework}
\end{figure*}
% We finally defined fairness metrics in TOD models as a robustness test on models but specifically focus on demographic perturbations.
% In this work, we follow \cite{sun2022computation} and \cite{qian2022perturbation} and hope models answer totally similar helpful response given demographic-perturbed user utterances. We use BLEU score which is the distance between generated text and groundtruth to define helpfulness for TOD models.
% For example, the response for 'I would like to find a movie for my mom.' should have similar helpfulness for 'I would like to find a movie for my dad.'.  
% Based on the concept, we proposed \textbf{generated-fairscore} that measure the \textbf{BLEU} difference between (original utterances, riginal groundtruth) and (perturbed utterances, perturbed groundtruth). To be more formal, asume we have TOD models $f_t$, original user utterance $u_t$, original response groundtruth $g_t$, perturbed user utterance $\widetilde{u_t}$, and perturbed response groundtruth $\widetilde{g_t}$. The model $f_t$ has bias if the BLEU score $BLEU(f_t(u_t), g_t) != BLEU(f_t(\widetilde{u_t}), \widetilde{g_t})$. With this concept, we define our generated fairscore as 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proposed Method}
\label{subsec:proposed_method}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
To get a more in-depth understanding of the biased responses, we propose a diagnosis method to attribute the bias to the potentially biased TOD components. We introduce the perturbation details in Section~\ref{subsubsec:perturbation} and describe the attribution procedure in Section~\ref{subsubsec:bias_attribution}.
% The motivation behind the method relies on measuring the distance between responses with original input and responses with perturbed input. Meanwhile, we also measure the distance improvements, which are the contributions by fixing the modules in the end-to-end TOD step by step.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Perturbation}
\label{subsubsec:perturbation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The proposed method requires perturbing the original input user utterances to measure the bias. We modified \citet{qian2022perturbation}'s perturbation algorithm to suit our scenario.

% In our proposed method, the first step is to perturb the input user utterances to measure the disparities. In order to maintain the consistency of dialogue, we employed and modified the algorithm from \cite{qian2022perturbation} to a suitable perturbation method.

Let $\SS$ be the original input dialogue dataset consisting of variable-length turn of dialogues, where $turn \in dialog$ is a turn in dialogue and $w$ is a word in $turn$ with demographic attribute $a_w$. We denote the attribute pair (source, target) as $(a_s, a_t) \in \mathcal{P}$, where $\mathcal{P} \subseteq \A \times \A$. $\A$ is the demographic attribute set.

% Let $\SS$ be the original input dialogue dataset consisting variable-length turn of dialogues, where $turn \in dialog$ is a turn in dialogue and $w$ is a word in $turn$ with demographic attribute $a_w$. We define an attribute pair (source, target) as $(a_s, a_t) \in \mathcal{P}$ where $\mathcal{P} \subseteq \A \times \A $ and $\A$ be a set of demographic attributes.

Algorithm~\ref{algo:DataCollection} describes the dialogue augmentation procedure. We first identify the set of perturbable words for each dialogue turn with the word lists. Note that each perturbable word's source and target attributes are also identified. We then sample a word from the collected perturbable words with target attributes $K$ and apply the perturbation to every dialogue turn. To ensure dialogue consistency, we perform the identical perturbation on dialogue states and database search results. Table~\ref{tab:generated_examples} shows the perturbed user utterances.
% The detail of the procedure of how we augmented the dialogue in the dataset is described in Algorithm~\ref{algo:DataCollection}.

% For each turn in dialogue, we first identify the set of perturbable demographic words with the word lists. We also identify each perturbable word's source and target attributes. Then we sample a perturbable word from the collected set of perturbable words with target attributes, $K$, and apply the perturbation to every turn in the dialogue. 
% To ensure dialogue consistency, we perform the same perturbation on the dialogue state and database search results containing the perturbable words. Table~\ref{tab:examples} shows the perturbed user utterances results.

\begin{algorithm}
\DontPrintSemicolon
 \textbf{Input:} dataset $\SS$, set of attribute pairs $\mathcal{P}_\text{d}$, dictionary of demographic words $\D_\text{d}$  \;
    
    \textbf{Initialize:} new dataset $\Stilde \leftarrow \emptyset$\;
    \For{dialog: $dialog \in \SS$}{
        new dialog $\widetilde{dialog} \leftarrow \emptyset$\;
        \For{turn:  $turn \in dialog$}{
        new turn $\widetilde{turn} \leftarrow turn$\;
        new $K \leftarrow \emptyset$\;
        \For{word $w \in turn  \cap \D_\text{d}$}{
            \For{ $(\cdot,t) \in \set{(a_s, a_t) \in \mathcal{P}_{\text{d}} | a_s = a_w, a_s \neq a_t}$}{
            $K \leftarrow K \cup \set{w, t}$\;
            }
        }
        }
        $(w, t) \sim \mathcal{U}(K)$\;
        \For{turn $turn \in dialog$}{
        $\widetilde{turn} \leftarrow$ \texttt{perturber(turn, w, t)}\;
        
        $\widetilde{dialog} \leftarrow \widetilde{dialog} \cup \widetilde{turn}$\
        }
        $\Stilde \leftarrow \Stilde \cup \set{\widetilde{s}}$\;
    }
    \textbf{Output:} $\Stilde$
   \caption{Data Augmentation via Demographic Perturbation}\label{algo:DataCollection}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Bias Attribution}
\label{subsubsec:bias_attribution}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As mentioned in Section~\ref{subsec:task-oriented_dialogue}, a TOD system usually consists of the following components: API call model, database (DB), and response generation model. All these components can cause biased responses toward different demographic attributes. When attributing the bias, we eliminate each component's influence on the bias by changing the component setting. After the setting of the component is updated, the change of the fairscore is attributed to the component. The attribution consists of three steps, we describe the details below. 
\begin{itemize}
    
    \item \textbf{Step 1 - Fairscore Evaluation:} In the beginning, we evaluate the fairscore by inputting a perturbed user utterance to the TOD system and get a fairscore of \textit{uttr'} based on generated responses. As shown in Figure~\ref{fig:framework}, the fairscore of $\tilde{uttr}$ is $0.23$.
    
    \item \textbf{Step 2 - Resolving DB Mismatch:} We then exclude DB search's influence on bias by resolving DB's mismatch issue. Though we can calculate the change of the fairscore and attribute the difference to the DB, it can be meaningless as we do not have the original dataset. That is, we do not know whether the perturbed API call can find necessary data from the original dataset. In Figure~\ref{fig:framework}, the fairscore of $\tilde{uttr}$ after this step is $0.18$.
    
    \item \textbf{Step 3 - API Call Adjustment:} In this step, we perturb the API call of \textit{uttr} and use the perturbed API call for the downstream components. The content of the perturbed API call should be semantically identical to the API call of \textit{uttr} but with different demographic attributes. In Figure~\ref{fig:framework}'s example, the change of the fairscore after the API call perturbation is $0.18 - 0.14 = 0.04$. After solving the mismatch problem in the previous step, the bias ($0.18$) comes from the API call model and the response generation model. Therefore, we can attribute the bias contribution $0.04$ and the bias contribution $0.14$ to the API call model and the response generation model, respectively.
    
    %After we solved the mismatch problem in the database we used, we aimed to solve the disparity in the API call module. To mitigate the influence of the API call module and measure the improvement in terms of fairscore. We simply perform the perturbation on the original API call result in figure xxx and use it as an alternative API call for the following downstream module to generate a response. With that said, since we perform the perturbation directly on the original API call module, the comparison of the original and perturbed pipeline are totally parallel. Parallel means that they are semantically similar but only have different demographics mentioned. We can expect an improvement after we make generated API call parallel in step 3 (0.14) and we attribute the improvement (0.18 - 0.14) as the bias contribution for API call module.

    % Response Module contribution: Although we have already fixed every module in the framework and aimed to make intermediate results parallel for the response generation module. We still observed that the fairscore was not zero (0.14). To explain the issue, we attribute the difference is the bias coming from the response generation module. (0 - 0.14)
    % Overall, after go through the whole diagnosis method mentioned above, we could receive an improvement for fixing each module: 0.04 for API call and 0.14 for response generation and it’s attribution for each module in terms of bias.


\end{itemize}





==> sections/gender_disparities.tex <==



==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}
Recent advances in machine learning have led conversational assistants such as Google Home, Alexa \cite{https://doi.org/10.48550/arxiv.1801.03604}, and Siri to become popular and essential in our daily life. However, models of conversational assistants can learn harmful societal biases from datasets, leading to biased model behavior.

Various existing works studied bias in open-domain dialogue systems. \citet{dinan-etal-2020-queens} investigated multiplayer text-based fantasy adventure dataset LIGHT \cite{urbanek-etal-2019-learning} and proposed a bias mitigation method by adding a control bin as a prompt during training. \citet{liu-etal-2020-gender} mitigated gender bias with a regularization method. \citet{sun2022computation} studied geographical fairness in TOD systems and proposed a new dataset to evaluate TOD's helpfulness toward different developing countries.

% With the power of machine learning, conversational assistants such as Google Home, Alexa, and Siri have become popular these years. They help solve people's daily requests by talking with them.
% However, the harmful societal bias and disparities also are learned from the dataset when people take advantage and pursue the performance of these models. 
% Previously, people have studied fairness and bias a lot in open-domain dialogue systems. \cite{dinan-etal-2020-queens} investigated multiplayer text-based fantasy adventure dataset LIGHT (\cite{urbanek-etal-2019-learning}) and proposed a new bias mitigation method by adding a control bin as a prompt during training.
% \cite{liu-etal-2020-gender} investigated the gender bias in open-domain dialogue datasets, and they proposed a regularization to mitigate bias. 
% On the other side, \cite{sun2022computation} studied geographical fairness in TOD systems. They proposed a new dataset to evaluate equal helpfulness given different developing countries in TOD systems.
\begin{figure}[htp!]
    \centering
    \includegraphics[width = \linewidth]{pics/example7.pdf}
    \caption{Language models can be biased toward specific demographic attributes. We propose a diagnosis method to attribute bias to the components of task-oriented dialogue systems.}
    \label{fig:example}
\end{figure}

Figure~\ref{fig:example} demonstrates the composition of a TOD system. A TOD system can be decomposed into three components: API call model, database, and response generation model. The example user utterances in Figure~\ref{fig:example} show that the TOD system is biased toward gender. In this case, all three components of the TOD system can contribute to the final biased behavior. However, existing works only studied the accumulated bias. To get a more in-depth understanding of the sources of bias, we propose a diagnosis method to attribute bias to each component of TOD systems. We believe the proposed attribution method can facilitate research on fairness mitigation.

% Traditional task-oriented dialogue (TOD) systems can be decomposed into several components: API Call, database, and response generation model. The previous works focus on bias measurement and mitigation in TOD systems. But no works are studying where bias comes from. It is important to know where bias comes from so that we can mitigate bias and start from the problem more efficiently.

% As shown in Figure~\ref{fig:example}, on the top side of the figure, the chatbot has different responses given requests for male and female psychiatrists in Fremont. In this situation, the gender disparity might be because the API call model generates biased results or the response generation model's bias. To solve this problem, we proposed a new diagnosis method to investigate the bias attribution of each model in TOD systems.

In this work, we first study fairness on well-known TOD datasets. Then, we attribute the societal bias of models trained with these well-known datasets to the TOD system's components. Unlike the hand-crafted bias measuring methods in previous works, our attribution is conducted by applying the perturber \cite{qian2022perturbation} to the whole dialogue. We propose a newly designed fairness metric to evaluate the bias by comparing original and perturbed user utterances. After measuring the accumulated bias, we update each component's setting to eliminate the resulting bias. The bias change after the component setting is updated can be regarded as the bias contribution of the component. By repeating this procedure, we can attribute the accumulated bias to each component of the TOD system.
% In this work, we first study fairness on the well-known TOD datasets that people usually use to train models. Second, we study the societal bias that models trained on these datasets. To measure the bias in TOD systems. Unlike previous works that measure bias with hand-crafted test cases. We aimed at combining the perturber \cite{qian2022perturbation} into our work to perturb whole dialogues. We also proposed a new evaluation metric that measures the bias based on the changes in generated responses given original and perturbed user requests.
% Finally, our diagnosis method could attribute the bias degree of each module by changing the components step by step of whole systems.
% Our bias attribution method covers three important demographic axes, gender, age, and race.
% In our experimental setup, we experimented with several transformer-based models with different pretrained methods.
We conduct experiments on several transformer-based models with different pretrained methods. Our experiments cover three essential demographic axes: gender, age, and race. The experimental results show that the bias of a TOD system mainly comes from the response generation model.
% The contributions of our work are as follows:
% \begin{itemize}
%     \item \textbf{Fairness in TOD}: We studied the societal bias, including age, race, and gender in Task-oriented dialogue systems.
%     \item \textbf{Bias Attribution method}: We proposed a new attribution method that help people find out the bias degree for each module in TOD systems.
% \end{itemize}













==> sections/related_works.tex <==
\section{Related Works}
% \textcolor{blue}{\paragraph{Fairness in Language Generation}
\subsection{Fairness in Language Generation}
Societal bias issues in natural language generation have drawn a lot of attention recently \cite{sheng2021societal}. We introduce two of them, bias evaluation and bias mitigation, in this section.
% Societal issues in Natural Language Generation have gained increasing attention recently \cite{sheng2021societal}, we would like to introduce two directions in this section: Bias evaluation and Bias mitigation. 

\citet{10.1162/tacl_a_00425} showed that traditional bias evaluation metrics, such as demographic parity \cite{10.1145/2090236.2090255} and equalized odds \cite{NIPS2016_9d268236}, are not applicable to text results. Therefore, discrete language generation results need dedicated evaluation methods. Researchers have proposed several methods to measure the fairness of language generation results. \citet{https://doi.org/10.48550/arxiv.2106.13219} and \citet{nadeem-etal-2021-stereoset} divided the bias evaluation methods into two categories: local bias-based and global bias-based. Local bias-based methods use hand-crafted templates to evaluate the fairness. For example, the template can be a sentence with some masked words. We can then evaluate the fairness by comparing the model's token probability of the masked words \cite{zhao-etal-2017-men, kurita-etal-2019-measuring, bordia-bowman-2019-identifying}. Global bias-based methods use multiple classifiers to evaluate the fairness by comparing the classification results of generated texts from various different perspectives. Previous works used regard ratio \cite{sheng2019woman, sheng-etal-2020-towards, 10.1145/3442188.3445924}, sentiment \cite{liu-etal-2020-mitigating, groenwold-etal-2020-investigating, huang-etal-2020-reducing, sheng2019woman, 10.1145/3442188.3445924, liu2019does}, offensive \cite{liu-etal-2020-mitigating}, and toxicity \cite{10.1145/3442188.3445924} as classifiers. In addition to off-the-shelf classifiers, existing works also analyzed word usage on generated texts. \citet{dinan-etal-2020-queens} measured the word count of the gender group (i.e., male, female) in the model's generated text; \citet{liu-etal-2020-mitigating, liu2019does} count the word frequency of ``career'' and ``family'' given male and female inputs. % For the bias evaluation metrics, since it's hard to measure discrete generated results with traditional algorithmic bias evaluation metrics \cite{10.1162/tacl_a_00425} (e.g., demographic parity \cite{10.1145/2090236.2090255}, equalized odds \cite{NIPS2016_9d268236}). 
% To measure fairness in the generation results, researchers proposed several methods that measure the model's generation performance \cite{https://doi.org/10.48550/arxiv.2106.13219, nadeem-etal-2021-stereoset}, which could be roughly categorized into two directions. In the first direction, people focus on model's next token probability given hand-crafted templates with similar semantics, but different demographics mentioned \cite{zhao-etal-2017-men, kurita-etal-2019-measuring, bordia-bowman-2019-identifying}. 
% \citep{https://doi.org/10.48550/arxiv.2105.14150} calculated dialogue state's entity bias given different domains on both generated dialogue states and dataset.
% On the other side, people can also measure fairness directly on models' generated results with various text evaluation metrics. For example, researchers used various classifiers to measure model-generated results: Regard ratio \cite{sheng2019woman, sheng-etal-2020-towards, 10.1145/3442188.3445924}, Sentiment \cite{liu-etal-2020-mitigating, groenwold-etal-2020-investigating, huang-etal-2020-reducing, sheng2019woman, 10.1145/3442188.3445924, liu2019does}, Offensive \cite{liu-etal-2020-mitigating}, Toxicity \cite{10.1145/3442188.3445924}. In addition to off-the-shelf classifier, people also measured word usage on generated texts:  \cite{dinan-etal-2020-queens} measured the gender groups (i.e., male, female) mentioned in model's generated text; \cite{liu-etal-2020-mitigating, liu2019does} detect the 'career' and 'family' word usages given male and female inputs.

For bias mitigation, an intuitive method is called Counterfactual Data Augmentation (CDA). People applied word-based augmentation that augmented all the demographics mentioned in texts, and trained models on the augmented data to equalize the word usage imbalance problem in the dataset to mitigate bias \cite{hall-maudslay-etal-2019-name, liu2019does, zmigrod-etal-2019-counterfactual}. In addition to CDA, there are various training-based methods to mitigate bias, for example, \citet{dinan-etal-2020-queens} finetune models with controllable prefixes to equalize the word usage for male and female. \citet{liu-etal-2020-mitigating} proposed a novel adversarial method that disentangles text into semantic and gender features to mitigate bias. \citet{https://doi.org/10.48550/arxiv.2106.13219} employed the concept of Null space projection \cite{may-etal-2019-measuring} to eliminate gender feature in models. More recently, \citet{sharma2022sensitive} used hand-crafted prompts \cite{li-liang-2021-prefix} to mitigate bias in machine translation. \citet{sheng-etal-2020-towards} also proposed to generate prompts to equalize gender and race's disparity in the dialogue generation task.

% \paragraph{End-to End Task-oriented Dialogue} 
\subsection{End-to-end Task-oriented Dialogue}
Task-Oriented Dialogue (TOD) systems help people resolve specific problems in domains such as restaurant booking and flight booking. TOD systems traditionally can be decomposed into several components: Natural Language Understanding, Dialogue State Tracking, Policy Learning, and Natural Language Generation. \cite{https://doi.org/10.48550/arxiv.2105.04387, liu-lane-2018-end}. Historically, these modules were trained individually \cite{DBLP:journals/corr/AsriHS16, DBLP:journals/corr/BordesW16, liu-lane-2018-end, lin2021zero}. However, individual components have the drawback of being non-differentiable. Pretrained large language models (LLMs) provide an end-to-end solution, and have been shown to not only resolve the aforementioned problems, but also improve the performance of TOD systems\cite{https://doi.org/10.48550/arxiv.2005.00796}. In this training manner, the user utterance, API call, and DB result are concatenated together and the model is trained autoregressively to generate the final response \cite{https://doi.org/10.48550/arxiv.2005.00796, ham-etal-2020-end, peng2020soloist, lin-etal-2020-mintl}. In this work, we followed the latter approach and trained end-to-end TOD systems with LLMs (GPT-2 \cite{radford2019language}, BART \cite{DBLP:journals/corr/abs-1910-13461}, and T5 \cite{2020t5}).

% \paragraph{Robustness Evaluation}
\subsection{Evaluation with Perturbation}
% Since the power of these large PLMs, people started including these powerful models to pursue the performance of their products. 

When we deploy LLMs to products, it is expected that lots of real and out-of-domain (OOD) issues exist, which can manifest in bias toward certain user groups \cite{ribeiro-etal-2020-beyond}. Previous approaches for evaluating the fairness of ML systems relied on hand-crafted perturbation examples, counterfactuals, or creating adversarial examples from scratch \cite{gardner-etal-2020-evaluating, https://doi.org/10.48550/arxiv.2004.09034, https://doi.org/10.48550/arxiv.1909.12434, xu-etal-2021-bot, ribeiro-etal-2020-beyond}. Recently, researchers have applied model-based methods to generate texts to influence model behavior \cite{wu-etal-2021-polyjuice, qian2022perturbation, wallace-etal-2019-universal, https://doi.org/10.48550/arxiv.2112.08321, https://doi.org/10.48550/arxiv.2010.12850, https://doi.org/10.48550/arxiv.2105.14150}. These prior works showed that model-based methods not only enhance the efficiency of test case generation, but also model-generated texts have higher performance in influencing and testing models' behavior.
